SOSELETO: A Unified Approach to Transfer Learning and Training with Noisy Labels

We present SOSELETO (SOurce SELEction for Target Optimization), a new method for exploiting a source dataset to solve a classification problem on a target dataset. SOSELETO is based on the following simple intuition: some source examples are more informative than others for the target problem. To capture this intuition, source samples are each given weights; these weights are solved for jointly with the source and target classification problems via a bilevel optimization scheme. The target therefore gets to choose the source samples which are most informative for its own classification task. Furthermore, the bilevel nature of the optimization acts as a kind of regularization on the target, mitigating overfitting. SOSELETO may be applied to both classic transfer learning, as well as the problem of training on datasets with noisy labels; we show state of the art results on both of these problems.

==> related.tex <==
\section{Related work}
\label{sec:related}

\smallpar{Transfer learning.} The most common techniques for transfer learning are feature extraction and fine-tuning, see for example \citet{donahue2014decaf} and \citet{girshick2014rich}, respectively.  An older survey of transfer learning techniques may be found in \cite{pan2010survey}.  Domain adaptation \cite{saenko2010adapting} is concerned with transferring knowledge when the source and target classes are the same.  Earlier techniques aligned the source and target via matching of feature space statistics \cite{tzeng2014deep,long2015learning}; subsequent work used adversarial methods to improve the domain adaptation performance \cite{ganin2015unsupervised,tzeng2015simultaneous,tzeng2017adversarial,hoffman2017cycada}.
%
In this paper, we are more interested in transfer learning where the source and target classes are different.  A series of recent papers \cite{long2017deep,pei2018multi,cao2018unsupervised,cao2018partial} address domain adaptation that is closer to our setting.  In particular, \cite{cao2018partial} examines ``partial transfer learning'',  the case in which there is partial overlap between source and target classes (particularly when the target classes are a subset of the source).  This setting is also dealt with in \cite{busto2017open}.
% 
Similar to SOSELETO, \cite{ge2017borrowing} propose selecting a portion of the source dataset. However, the selection is done prior to training and not performed in an end-to-end fashion.
%\cite{ge2017borrowing} examine the scenario where the source and target classes are completely different.  Similar to SOSELETO, they propose selecting a portion of the source dataset.  However, the selection is not performed in an end-to-end fashion, as in SOSELETO; rather, selection is performed prior to training, by finding source examples which are similar to the target dataset, where similarity is measured by using filter bank descriptors.
In \cite{luo2017label}, an adversarial loss is utilized to align the source and the target representations in a few-shot setting. 

%Another recent work of interest is \cite{luo2017label}, which focuses on a slightly different scenario: the target consists of a very small number of labelled examples (i.e.~the few-shot regime), but a very large number of unlabelled examples.  Training is achieved via an adversarial loss to align the source and the target representations, and a special entropy-based loss for the unlabelled part of the data.

\smallpar{Instance reweighting} is a well studied technique for domain adaptation, demonstrated e.g. in Covariate Shift methods \citep{shimodaira2000improving, sugiyama2007covariate, sugiyama2008direct}. While in these works, the source and target label spaces are the same, we allow them to be different -- even entirely non-overlapping. Crucially, we do not make assumptions on the similarity of the \textit{distributions} nor do we explicitly optimize for it. The same distinction applies for the recent work of \cite{yan2017mind}, and for the partial overlap assumption of \cite{zhang2018importance}. In addition, these two works propose an \textit{unsupervised} approach, whereas our proposed method is completely supervised. %Covariate shift determines the weighting for an instance as the ratio of its probability of being in the training set and being in the prediction set. Consequently, the feature vectors are used in re-weighting, regardless of their labels. This renders covariate shift unsuitable for handling noisy labels. Our re-weighing scheme is instead gradient-based and as we show next performs well in this task.

\smallpar{Classification with noisy labels} is a longstanding problem in the machine learning literature, see the review paper \cite{frenay2014classification}. Within the realm of deep learning, it has been observed that with sufficiently large data, learning with label noise -- without modification to the learning algorithms -- actually leads to reasonably high accuracy \citep{krause2016unreasonable,sun2017revisiting,rolnick2017deep,drory2018resistance}. We consider the setting where the large noisy dataset is accompanied by a small clean dataset. \citet{sukhbaatar2014training} introduced a noise layer into the CNN that adapts the output to align with the noisy label distribution. \citet{xiao2015learning} proposed to predict simultaneously the clean label and the type of noise; 
%use a more general noise model, in which the clean label, noisy label, noise type, and image are jointly specified by a probabilistic graphical model.  Both the clean label and the type of noise must be inferred given the image, in this case by two separate CNNs.
\cite{li2017learning} consider the same setting, but with additional information in the form of a knowledge graph on labels.
%
%Other recent work on label noise includes \cite{rolnick2017deep}, which shows that adding many copies of an image with noisy labels to a clean dataset barely dents performance;
\cite{malach2017decoupling} conditioned the gradient propagation on the agreement of two separate networks. 
%in which two separate networks are simultaneously trained, and a sample only contributes to the gradient descent step if there is disagreement between the networks (if there is agreement, that probably means the label is wrong); and \cite{drory2018resistance}, which analyzes theoretically the situations in which CNNs are more and less resistant to noise. 
\cite{liu2016classification,yu2017transfer} combine ideas of learning with label noise with instance reweighting.

%\smallpar{Bilevel optimization}  A branch of mathematical programming, bilevel optimization has been extensively studied within this community \cite{colson2007overview,bard2013practical}.  For recent developments, readers are referred to the review paper \cite{sinha2018review}.  Bilevel optimization has been used occasionally in both machine learning, e.g.~\cite{bennett2006model,bennett2008bilevel} and computer vision, e.g.~\cite{ochs2015bilevel}.  In this context, it is worth mentioning the recent work of \cite{yang2017shape}, which solves the shape from shading problem without using an external shape dataset.  They simultaneously generate complex shapes from primitives and train on these shapes; while the formulation is different, the method has the flavor of a bilevel optimization framework.

%\smallpar{Bilevel optimization} problems have a nested structure: the interior level is a standard optimization problem; and the exterior level is an optimization problem where the objective is a function of the optimal arguments from the interior level.  A branch of mathematical programming, bilevel optimization has been extensively studied within this community \cite{colson2007overview,bard2013practical}.  For recent developments, readers are referred to the review paper \cite{sinha2018review}.  %Bilevel optimization has been used in both machine learning, e.g.~\cite{bennett2006model,bennett2008bilevel} and computer vision, e.g.~\cite{ochs2015bilevel}.
